PoM: A Linear-Time Replacement for Attention with the Polynomial Mixer

This paper introduces the Polynomial Mixer (PoM), a novel token mixing mechanism with linear complexity that serves as a drop-in replacement for self-attention. PoM aggregates input tokens into a compact representation through a learned polynomial function, from which each token retrieves contextual information. We prove that PoM satisfies the contextual mapping property, ensuring that transformers equipped with PoM remain universal sequence-to-sequence approximators. We replace standard self-attention with PoM across five diverse domains: text generation, handwritten text recognition, image generation, 3D modeling, and Earth observation. PoM matches the performance of attention-based models while drastically reducing computational cost when working with long sequences. The code is available at https://github.com/davidpicard/pom.

==> figures/diff_speed.tex <==
\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{
\begin{tikzpicture}
    \begin{axis}[
        width=\columnwidth,
        height=0.8\columnwidth,
        xlabel={Image resolution},
        ylabel={Time in second/image},
        ymode=log,
        xtick={256, 1024, 2048, 4096},
        grid=both,
        grid style={line width=.1pt, draw=gray!10},
        major grid style={line width=.2pt, draw=gray!30},
        xmin=0, xmax=4352,
        ymin=0.01, ymax=6,
        legend style={at={(0.98,0.02)}, anchor=south east, font=\footnotesize},
        legend cell align=left,
        every axis plot/.append style={very thick}
    ]

    \addplot[color=blue!70, mark=o] coordinates {
        (256, 0.038862082336563616)
        (384, 0.03905078684678301)
        (512, 0.04221228306181729)
        (768, 0.05795255176257342)
        (1024, 0.09442358191823587)
        (1536, 0.17702449211617932)
        (2048, 0.29645248390734197)
        (3072, 0.6015695175528526)
        (4096, 1.0516053920192645)
    };
    \addlegendentry{PoM forward+backward}

    \addplot[color=blue!70, mark=o, dashed, mark options={solid}] coordinates {
        (256, 0.015069471425376832)
        (384, 0.015871938960626723)
        (512, 0.0189380434085615)
        (768, 0.02909953865222633)
        (1024, 0.04561432354385033)
        (1536, 0.080849758409895)
        (2048, 0.13602926889434458)
        (3072, 0.2696375051792711)
        (4096, 0.47321898558177056)

    };
    \addlegendentry{PoM forward}

    \addplot[color=orange!80, mark=square, dashed, mark options={solid}] coordinates {
        (256, 0.010657461867667735)
        (384, 0.012714778319932521)
        (512, 0.014707973287440836)
        (768, 0.02519212323939428)
        (1024, 0.037897837879136205)
        (1536, 0.08845603726571426)
        (2048, 0.18336747443769127)
        (3072, 0.6122184240771458)
        (4096, 1.6892871374706737)
    };
    \addlegendentry{MHA forward}
    
    \addplot[color=orange!80, mark=square] coordinates {
        (256, 0.03005698923021555)
        (384, 0.032288018770050254)
        (512, 0.03444906664080918)
        (768, 0.05218656954821199)
        (1024, 0.08344621217343956)
        (1536, 0.21130420179106296)
        (2048, 0.4523333204118535)
        (3072, 1.639214531343896)
        (4096, 4.577012917282991)
    };
    \addlegendentry{MHA forward+backward}

    \end{axis}
\end{tikzpicture}
    }
    \caption{\textbf{Comparison between the speed of PoM and Multi-Head Attention (MHA) in the same DiT-XL/2 architecture for different image resolutions.} We use an H100 GPU and compute the average time on 100 synthetic training batches to perform the forward or forward+backward passes. We use synthetic data to remove the influence from data loading.}
    \label{fig:enter-label}
\end{figure}

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}




